PySS3: A Python package implementing a novel text classifier with visualization tools for Explainable AI

A recently introduced text classifier, called SS3, has obtained state-of-the-art performance on the CLEF's eRisk tasks. SS3 was created to deal with risk detection over text streams and, therefore, not only supports incremental training and classification but also can visually explain its rationale. However, little attention has been paid to the potential use of SS3 as a general classifier. We believe this could be due to the unavailability of an open-source implementation of SS3. In this work, we introduce PySS3, a package that implements SS3 and also comes with visualization tools that allow researchers to deploy robust, explainable, and trusty machine learning models for text classification.

==> minted/Makefile <==
TEXFLAGS = -e '$$pdflatex=q/pdflatex %O -shell-escape %S/' -pdf
LATEXMK = latexmk

PACKAGE = minted.dtx \
		  minted.ins \
		  minted.pdf \
		  README \
		  Makefile

.PHONY: minted all doc dist clean cleanall

minted: minted.sty

doc: minted.pdf

all: minted doc

minted.sty: minted.ins minted.dtx
	tex minted.ins

minted.pdf: minted.sty minted.gls minted.dtx
	$(LATEXMK) $(TEXFLAGS) minted.dtx

minted.gls: minted.glo
	makeindex -s gglo.ist -o minted.gls minted.glo

minted.glo: minted.dtx minted.sty
	$(LATEXMK) $(TEXFLAGS) minted.dtx

dist: $(PACKAGE)
	@$(RM) minted.zip
	@zip minted-$(shell grep '^\\ProvidesPackage' < minted.sty | grep -o '\<v[[:digit:]]*\.[[:digit:]]*\>').zip $(PACKAGE)

clean:
	@$(RM) *.aux *.log *.out *.toc *.fdb_latexmk *.ilg *.glo *.gls *.lol

cleanall: clean
	@$(RM) minted.sty minted.zip

